Deep-ELA: Deep Exploratory Landscape Analysis with Self-Supervised Pretrained Transformers for Single- and Multi-Objective Continuous Optimization Problems

In many recent works, the potential of Exploratory Landscape Analysis (ELA) features to numerically characterize, in particular, single-objective continuous optimization problems has been demonstrated. These numerical features provide the input for all kinds of machine learning tasks on continuous optimization problems, ranging, i.a., from High-level Property Prediction to Automated Algorithm Selection and Automated Algorithm Configuration. Without ELA features, analyzing and understanding the characteristics of single-objective continuous optimization problems is -- to the best of our knowledge -- very limited. Yet, despite their usefulness, as demonstrated in several past works, ELA features suffer from several drawbacks. These include, in particular, (1.) a strong correlation between multiple features, as well as (2.) its very limited applicability to multi-objective continuous optimization problems. As a remedy, recent works proposed deep learning-based approaches as alternatives to ELA. In these works, e.g., point-cloud transformers were used to characterize an optimization problem's fitness landscape. However, these approaches require a large amount of labeled training data. Within this work, we propose a hybrid approach, Deep-ELA, which combines (the benefits of) deep learning and ELA features. Specifically, we pre-trained four transformers on millions of randomly generated optimization problems to learn deep representations of the landscapes of continuous single- and multi-objective optimization problems. Our proposed framework can either be used out-of-the-box for analyzing single- and multi-objective continuous optimization problems, or subsequently fine-tuned to various tasks focussing on algorithm behavior and problem understanding.

==> tables/bbob_hlp_full.tex <==
\tiny
\begin{tabular}{@{}lllllllll@{}}
	\toprule
	{\bf BBOB Function} & {\bf Multim.} & {\bf Global Str.} & {\bf Separab.} & {\bf Var. Sc.} & {\bf Search Sp.} & {\bf Basin Size} & {\bf Gl.-Loc.} & {\bf Funnel}\\\midrule
    1: Sphere & none & none & high & none & high & none & none & yes \\
    2: Ellipsoidal separable & none & none & high & high & high & none & none & yes  \\
    3: Rastrigin separable & high & strong & high & low & high & low & yes & yes \\
    4: B\"uche-Rastrigin & high & strong & high & low & high & med. & yes & yes \\
    5: Linear Slope & none & none & high & none & high & none & none & yes \\ \midrule
    6: Attractive Sector & none & none & none & low & med. & none & none & yes \\
    7: Step Ellipsoidal & none & none & none & low & high & none & none & yes  \\
    8: Rosenbrock & low & none & none & none & med. & low & yes & yes\\
    9: Rosenbrock rotated & low & none & none & none & med. & low & yes & yes\\ \midrule
    10: Ellipsoidal high conditioned & none & none & none & high & high & none & none & yes \\
    11: Discus & none & none & none & high & high & none & none & yes\\
    12: Bent Cigar & none & none & none & high & high & none & none & yes\\
    13: Sharp Ridge & none & none & none & low & med. & none & none  & yes\\
    14: Different Powers & none & none & none & low & med. & none & none & yes\\ \midrule
    15: Rastrigin multimodal & high & strong & none & low & high & low & yes & yes\\
    16: Weierstrass & high & med. & none & med. & high & med. & yes & none\\
    17: Schaffer F7 & high & med. & none & low & med. & med. & yes & yes\\
    18: Schaffer F7 moderately ill-cond. & high & med. & none & high & med. & med. & yes & yes\\
    19: Griewank-Rosenbrock & high & strong & none & none & high & low & yes & yes\\ \midrule
    20: Schwefel & med. & deceptive & none & none & high & low & yes & yes\\
    21: Gallagher 101 Peaks & med. & none & none & med. & high & med. & yes & none\\
    22: Gallagher 21 Peaks & low & none & none & med. & high & med. & yes & none\\
    23: Katsuura & high & none & none & none & high & low & yes & none\\
    24: Lunacek bi-Rastrigin & high & weak & none & low & high & low & yes & yes\\\midrule
\end{tabular}

==> tables/results_mo_as_full.tex <==
\small
\begin{tabular}{lrrrrrrrr}
\toprule
 & \multicolumn{2}{c|}{Large (25$d$)} & \multicolumn{2}{c|}{Large (50$d$)} & \multicolumn{2}{c|}{Medium (25$d$)} & \multicolumn{2}{c}{Medium (50$d$)} \\
Function & $k$NN & RF & $k$NN & RF & $k$NN & RF & $k$NN & RF \\
\midrule[1pt]
BiObjBBOB1 & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} \\
BiObjBBOB2 & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} \\
BiObjBBOB3 & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} \\
\midrule[1pt]
DTLZ1 & 0.600 & 0.000 & \textbf{1.000} & 0.000 & \textbf{1.000} & 0.200 & \textbf{1.000} & 0.200 \\
DTLZ2 & \textbf{1.000} & 0.600 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.800 & \textbf{1.000} & \textbf{1.000} \\
DTLZ3 & 0.800 & 0.200 & \textbf{1.000} & 0.600 & \textbf{1.000} & 0.000 & \textbf{1.000} & 0.800 \\
DTLZ4 & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} \\
DTLZ5 & \textbf{1.000} & 0.600 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.800 & \textbf{1.000} & \textbf{1.000} \\
DTLZ6 & \textbf{1.000} & 0.600 & \textbf{1.000} & 0.800 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
DTLZ7 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.877 & \textbf{1.000} & 0.754 \\
\midrule[1pt]
MMF1 & \textbf{1.000} & 0.119 & \textbf{1.000} & 0.459 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
MMF10 & \textbf{1.000} & 0.400 & \textbf{1.000} & 0.800 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
MMF11 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
MMF12 & 0.000 & 0.000 & 0.200 & 0.000 & 0.000 & 0.123 & \textbf{1.000} & 0.246 \\
MMF14 & 0.391 & 0.191 & 0.797 & 0.594 & 0.797 & 0.594 & \textbf{1.000} & \textbf{1.000} \\
MMF14a & \textbf{1.000} & 0.615 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.815 & \textbf{1.000} & \textbf{1.000} \\
MMF15 & 0.763 & 0.442 & 0.763 & 0.921 & 0.921 & \textbf{1.000} & \textbf{1.000} & 0.842 \\
MMF15a & 0.907 & 0.615 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.907 & \textbf{1.000} & \textbf{1.000} \\
MMF1e & \textbf{1.000} & 0.000 & \textbf{1.000} & 0.000 & \textbf{1.000} & 0.200 & \textbf{1.000} & 0.600 \\
MMF1z & \textbf{1.000} & 0.173 & \textbf{1.000} & 0.373 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
MMF2 & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} \\
MMF3 & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} \\
MMF4 & \textbf{1.000} & 0.200 & \textbf{1.000} & 0.800 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
MMF5 & \textbf{1.000} & 0.087 & \textbf{1.000} & 0.087 & \textbf{1.000} & 0.774 & \textbf{1.000} & 0.887 \\
MMF6 & \textbf{1.000} & 0.363 & \textbf{1.000} & 0.563 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
MMF7 & \textbf{1.000} & 0.200 & \textbf{1.000} & 0.600 & \textbf{1.000} & 0.307 & \textbf{1.000} & \textbf{1.000} \\
MMF8 & \textbf{1.000} & 0.000 & \textbf{1.000} & 0.400 & \textbf{1.000} & 0.400 & \textbf{1.000} & \textbf{1.000} \\
MMF9 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.803 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.901 \\
\midrule[1pt]
ZDT1 & \textbf{1.000} & 0.765 & \textbf{1.000} & 0.765 & \textbf{1.000} & 0.800 & \textbf{1.000} & 0.882 \\
ZDT2 & -3.796 & -2.837 & -3.796 & \textbf{1.000} & 0.041 & -1.877 & -0.918 & 0.800 \\
ZDT3 & \textbf{1.000} & 0.800 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.800 \\
ZDT4 & 0.400 & 0.000 & \textbf{1.000} & 0.279 & 0.400 & 0.000 & \textbf{1.000} & 0.638 \\
ZDT6 & \textbf{1.000} & 0.000 & \textbf{1.000} & 0.200 & \textbf{1.000} & 0.200 & \textbf{1.000} & 0.800 \\
\bottomrule
\end{tabular}
